BDD100K: A Diverse Driving Dataset for Heterogeneous Multitask Learning

Datasets drive vision progress, yet existing driving datasets are impoverished in terms of visual content and supported tasks to study multitask learning for autonomous driving. Researchers are usually constrained to study a small set of problems on one dataset, while real-world computer vision applications require performing tasks of various complexities. We construct BDD100K, the largest driving video dataset with 100K videos and 10 tasks to evaluate the exciting progress of image recognition algorithms on autonomous driving. The dataset possesses geographic, environmental, and weather diversity, which is useful for training models that are less likely to be surprised by new conditions. Based on this diverse dataset, we build a benchmark for heterogeneous multitask learning and study how to solve the tasks together. Our experiments show that special training strategies are needed for existing models to perform such heterogeneous tasks. BDD100K opens the door for future studies in this important venue.

==> tool.tex <==

Our goal is to design a versatile and scalable annotation tooling that is suitable for all kinds of annotations needed in a driving database, such as bounding box, semantic instance segmentation, and lane detection. Many open source annotation tools are targeted to one specific task, such as single object classification or vehicle/pedestrian detection, however, no existing open source tool is available to support various types of annotations for such a large driving database. Also, in order to have an extensive collection of images annotated with maximum efficiency, the annotation work must be easily accessible to workers, the annotation progress needs to be monitorable, and concurrent annotation sessions need to be supported. 

To satisfy these requirements, we design an efficient labeling system that is sufficient for the annotation of a large driving video database. First of all, the system is adaptable so that it would allow the practice of various kinds of annotation work such as bounding box and region annotation. Secondly, the system aims to make the annotation process as seamless and user-friendly as possible. Besides, we choose to implement the annotation system as a web-based tool so that it can be simply accessed through a web browser without installation. 
% The SaaS (Software as a Service) model we adopted safely stores all data in cloud, allows groups to share and collaborate on data concurrently, and simplifies the upgrade processes for developers so that user feedback could be responded in a fast manner.
Figure~\ref{fig:tool_system} (a) shows an overview of our system. In this section, we will describe the details and evaluate the efficiency of our annotation tool.

\begin{figure*}[htp]
  \centering
  \begin{tabular}{cc}
         \includegraphics[height=1.3in]{images/workflow.pdf}
 &   \includegraphics[height=1.3in]{images/bbox_tool.jpg} \\ 
 (a) Labeling tool workflow diagram. & (b) Bounding box labeling tool.
  \end{tabular}
  % \vspace{-5mm}
  \caption{Back-end and front-end of our labeling system}
  \label{fig:tool_system}
\end{figure*}


\subsection{Box Annotation}

% In this section, we discuss the bounding box annotation interface shown in Fig \ref{fig:tool_system} (b), which was used to annotate the 100k driving dataset.

% The annotation tool design emphasizes simplicity and ease of use. Annotators can draw and adjust bounding boxes tightly around the objects by using a simple "click and drag" action. On the left side is a drop-down menu that list all label categories as well as options to add attributes to a category, such as a light color for traffic lights. We observed that multiple bounding boxes of the same object often occur together, such as a group of cars or a group of pedestrians. Thus, the label category in these group situations are assumed to be the same in order to avoid the necessity of re-assigning the same label at each annotation. This way, annotators are able to continuously create new bounding boxes by dragging over the image and matching the selection with options displayed on a left sidebar. Another open annotation tool, LabelMe\cite{labelme} displays a pop-up dialog bubble and requests user to enter names upon completion of every label. In contrast to LabelMe, our strategy of label assignment was preferred by annotators and resulted in higher efficiency in labeling our dataset. Once an annotater finishes an image, the resulting work is automatically stored on the server. The resulting annotations are immediately available for download and can be viewed by concurrent annotators who visit the same web page. Concurrency is especially important for the verification stage when other annotators would inspect and correct any mislabeled objects in the same task. We also provided an instruction/guideline page to address corner cases and provide examples.

An interface example is shown in Fig.~\ref{fig:tool_system} (b). As a novel feature of our tool, suggestions on the category of a bounding box can be provided to annotators by using the outputs from an object detection model. After obtaining the annotations of the full 55k video clips, we trained a Fast-RCNN object detection model with IoU of 0.6. We set up the system by uploading the model outputs as initial annotations and ask annotators to complete the annotation by adjusting or adding new bounding boxes. An experiment was conducted to evaluate the efficiency of the semi-automatic system, which integrates outputs from object detection models with the manual system from only human inputs. Annotators were asked to draw bounding boxes around all objects of 10 given categories in 2,000 images using the two different systems, then record the time spent on operating each bounding box. As shown in Fig. \ref{fig:time}(a), the object detector is able to label 40\% of bounding boxes at a minimal cost. On average, the time of drawing and adjusting each bounding box is reduced by 60\%. Our study shows that our proposed semi-automatic system outperforms the manual process. To provide ground truth for future study of semi-automatic labeling systems, all the labeled provided in this paper are labeled manually.

\begin{figure}[htp]
  \centering
  \begin{tabular}{cc}
       \includegraphics[height=0.92in]{images/time.png} &
       \includegraphics[height=1in]{images/copy_border.png} \\
       (a) & (b)
  \end{tabular}
  
  \caption{(a) Distribution of time in seconds spent on drawing a new bounding box and adjusting a bounding box suggested by the object detection model. The histogram illustrates the percentage of bounding boxes drawn in time represented on the horizontal axis. (b) Distribution of time in seconds spent on drawing a polygon one by one, and using copying boundaries. By using this technique, the time is reduced significantly.}
  \label{fig:time}
\end{figure}

\subsection{Region Annotation}

%This section explains 
%
The region annotation interface is used to annotate region or boundary information, such as semantic segmentation, drivable area, and lane markings. To support fine and quick annotations, techniques similar to~\cite{labelme,vatic,opensurfaces}, such as a local magnifier, zoom in/out, and keyboard shortcuts, are implemented. To further facilitate the accuracy and effectiveness of annotation processes, we also introduce several innovative features, which outperform previous methods in providing finer and quicker annotation tooling. 

\minisection{Bezier curve}. To fit curved boundaries, we provide the option to draw parametric Bezier curves. Annotators can easily change any line segment to a cubic Bezier curve. By adjusting the shape of the curves, annotators could fit labels to objects with much higher accuracy and efficiency. As shown in Fig.~\ref{fig:bezier}, Bezier curve has apparent smoothness, compared with many dispersed clicks on a curved boundary.

\begin{figure}[htp]
  \centering
  \begin{tabular}{cc}
 \includegraphics[width=0.45\linewidth]{images/beizer/beizer_without.png} &
 \includegraphics[width=0.45\linewidth]{images/beizer/beizer_with.png} \\
 (a) Polygon with dispersed clicks. &  (b) Polygon using Beizer curves.
  \end{tabular}
  \caption{Compared to dispersed clicks in (a), Beizer curve in (b) provides us with more smoothness and less operations. The vertices connected by dashed lines are control points.}
  \label{fig:bezier}
\end{figure}

\minisection{Copy shared boundaries}. In tasks such as segmentation annotations, there are usually many objects to be labeled in an image. As shown in Fig~\ref{fig:border_example}, objects share boundaries with their neighbors. To avoid drawing the same boundaries repeatedly, we introduce the function to automatically duplicate shared boundaries and make it possible for a polygon to share boundaries with its neighbors. 

\begin{figure}[htp]
  \centering
  \begin{tabular}{ccc}
  \includegraphics[width=0.33\linewidth]{images/border_example.jpg}
  \includegraphics[width=0.33\linewidth]{images/border_example2.jpg}
  \includegraphics[width=0.33\linewidth]{images/border_example5.jpg}
  \caption{Polygons with shared boundaries.}
  \label{fig:border_example}
  \end{tabular}
\end{figure}

For example, when drawing a polygon A, if A's boundary partly overlaps with polygon B, which has already been drawn, the annotator can let the system automatically generate the shared boundary by clicking on two desired endpoints. In addition, adequate visual feedback is also implemented to smooth out the annotation process. The copy shared boundary feature not only provides unique and cleaner boundaries between adjacent objects, but also reduces the annotation time significantly. According to the our user study, in which annotators were asked to label 20 images with 842 polygons, the time to draw a polygon was reduced by 36\% on average when using this technique as shown in Fig.~\ref{fig:time}(b).


% \minisection{Encapsulated regions}. There are some cases in which a region should be drawn inside of another, such as windows and the building they belonging to. And when we want to adjust the shape of the encapsulated one, the outsider's shape can be also changed at the same time.

% \minisection{Link separated regions}. In some cases, there are several separated regions belonging to the same object. Linking them together is very meaningful for instance segmentation. So we also introduce the option to link separated regions together so that they can have the same instance id.

\subsection{Extensibility}

Vision tasks are mostly about regrouping pixels on the images and assigning semantic meanings to them. For example, when only the object location and extent are needed, bounding boxes are easier to annotate and recognize. Therefore, we provide operations that can be used for labeling different tasks and we provide that options for the system user to configure the semantics of the targeted regions. We study this extensibility by labeling large-scale real-world data with distinct types of annotations, which will be discussed in the following section.
